Subtyping for F-Bounded Quantifiers and Equirecursive Types (Extended Version)

This paper defines a notion of binding trees that provide a suitable model for second-order type systems with F-bounded quantifiers and equirecursive types. It defines a notion of regular binding trees that correspond in the right way to notions of regularity in the first-order case. It defines a notion of subtyping on these trees and proves various properties of the subtyping relation. It defines a mapping from types to trees and shows that types produce regular binding trees. It presents a set of type equality and subtyping rules, and proves them sound and complete with respect to the tree interpretation. It defines a notion of binding-tree automata and how these generate regular binding trees. It gives a polynomial-time algorithm for deciding when two automata's trees are in the subtyping relation.

==> defs.tex <==
\usepackage{xspace}
\newcommand{\etc}{\textit{et cetera\/}}
\usepackage{amsfonts}
\usepackage{amssymb}
\newcommand{\omitthis}[1]{}
\newcommand{\etal}{et al.\xspace}
%%% Metanotation
\newtheorem{dfn}{Definition}[section]
\newcommand{\dom}[1]{\mathrm{dom}(#1)}
\newcommand{\litset}[1]{\{#1\}}
\newcommand{\fix}[1]{\mathrm{fix}(#1)}
\newcommand{\IF}{\Leftarrow}
\newcommand{\IFF}{\Leftrightarrow}
\newcommand{\implies}{\Rightarrow}
\newcommand{\IN}[2]{\mathrm{in}_{#1}(#2)}
\newcommand{\kw}[1]{\mathsf{#1}}
\newcommand{\modelitem}[1]{{\it #1}}
\newcommand{\modelfn}[1]{{\rm #1}}
\newcommand{\nat}{{\mathbb N}}
\newcommand{\tfun}{\rightarrow}
\newcommand{\pfun}{\rightharpoonup}
\newcommand{\partialbij}{\leftrightharpoons}
\newenvironment{prf}{{\bf Proof:}\hspace*{0.5em}}{\hspace*{\fill}\qed}
\newenvironment{prfof}[1]{{\bf Proof of #1:}\hspace*{0.5em}}{\hspace*{\fill}\qed}
%\newcommand{\qed}{\mbox{\ \ }\hfill $\Box$ \medskip}
\newcommand{\reason}[1]{\quad\langle\hbox{#1}\rangle}
\newcommand{\sepbar}{\mathrel|}
\newcommand{\subst}[2]{#1\{#2\}}
\newcommand{\subtype}{\le}
\newenvironment{thm}{\begin{theorem}}{\end{theorem}}
\newenvironment{lem}{\begin{lemma}}{\end{lemma}}
%\newtheorem{thm}{Theorem}[section]
%\newtheorem{cor}[thm]{Corollary}
%\newtheorem{lem}[thm]{Lemma}
\newcommand{\var}{\phi}
\newcommand{\Var}{\mathit{Var}}
\newcommand{\bnfdef}{::=}
\newcommand{\bnfalt}{\mathrel|}
\newcommand{\ftv}[1]{\mathit{ftv}(#1)}
\newcommand{\rn}[1]{\textsc{#1}}
\newcommand{\last}[1]{\mathit{last}(#1)}
%%% Notation
\newcommand{\shift}[2]{\mathit{shift}(#1,#2)}
\newcommand{\fun}{\mathord{\rightarrow}}
% Tree Stuff
\newcommand{\Tree}{\mathit{Tree}}
\newcommand{\trvar}[1]{\mathrm{var}(#1)}
\newcommand{\trfun}[2]{#1\fun#2}
\newcommand{\trall}[2]{\forall#1.#2}
\newcommand{\bind}[2]{\mathit{bind}(#1,#2)}
\newcommand{\BSet}{\mathit{BSet}}
\newcommand{\subtree}[2]{\mathit{subtree}(#1,#2)}
\newcommand{\promotesto}[1]{\hookrightarrow_{#1}}
\newcommand{\sbtprop}[4]{\mathit{bst}(#1,#2,#3,#4)}
\newcommand{\LEFT}{\kw{L}}
\newcommand{\RIGHT}{\kw{R}}
\newcommand{\SHIFT}{\kw{S}}
\newcommand{\dropshifts}[1]{\mathit{ds}(#1)}
\newcommand{\nodelabel}[2]{\mathit{NL}(#1,#2)}
\newcommand{\bstr}[3]{\mathit{bstr}_{#1}(#2,#3)}
\newcommand{\fails}{\kw{F}}
\newcommand{\complete}{\kw{C}}
\newcommand{\trypromote}[4]{\mathit{tryp}_{#1}(#2,#3,#4)}
\newcommand{\pathresult}[2]{\mathit{pr}_{#1}(#2)}
\newcommand{\pmstart}[1]{\mathit{pmi}(#1)}
\newcommand{\pmstartec}[1]{\mathit{pmiec}(#1)}
\newcommand{\eqclass}[2]{\mathit{eqc}_{#1}(#2)}
\newcommand{\prmap}[1]{\mathit{pmf}(#1)}
\newcommand{\forbid}[2]{\mathit{forbid}(#1,#2)}
\newcommand{\eqst}[1]{\mathit{eqst}(#1)}
\newcommand{\fvar}[1]{\kw{fv}(#1)}
\newcommand{\bvar}[2]{\kw{bv}(#1,#2)}
\newcommand{\bounds}[2]{\mathit{bounds}(#1,#2)}
\newcommand{\trfv}[1]{\mathit{fv}(#1)}
\newcommand{\openvars}[2]{\mathit{open}_{#1}(#2)}
% Type Stuff
\newcommand{\TVar}{\mathit{Var}}
\newcommand{\Type}{\mathit{Type}}
\newcommand{\tyfun}[2]{#1\fun#2}
\newcommand{\tyall}[3]{\forall#1\le#2.#3}
\newcommand{\rec}[2]{\kw{rec}\;#1.#2}
\newcommand{\scontract}[2]{#1\downarrow#2}
\newcommand{\Env}{\mathit{Env}}
\newcommand{\env}{\eta}
\newcommand{\treeof}[2]{\mathit{treeof}(#1)_{#2}}
\newcommand{\typeof}[2]{\mathit{typeof}_{#1}(#2)}
\newcommand{\typol}[3]{#1\{#2^{#3}\}}
\newcommand{\tje}[2]{\vdash#1=#2}
\newcommand{\tjs}[3]{#1\vdash#2\le#3}
\newcommand{\tjsv}[4]{#1\vdash#2\le^{#3}#4}
\newcommand{\tyfv}[1]{\mathit{fv}(#1)}
\newcommand{\automataof}[2]{\mathit{automataof}_{#1}(#2)}
% Automata Stuff
\newcommand{\lf}{{\it lf}}
\newcommand{\promote}[2]{\mathit{promote}_{#1}(#2)}
\newcommand{\matches}[2]{\mathit{matches}_{#1}(#2)}
\newcommand{\subtypeautomata}[1]{\mathit{subtype}(#1)}
\newcommand{\subtreeta}[3]{\mathit{subtree}_{#1}(#2,#3)}
\newcommand{\ndidst}[2]{\mathit{ni2s}_{#1}(#2)}
\newcommand{\scs}[2]{\mathit{scs}_{#1}(#2)}
\newcommand{\cbij}[1]{\mathit{cbij}(#1)}
\newcommand{\stst}[2]{\mathit{ss}_{#1}(#2)}
\newcommand{\esst}[2]{\mathit{ess}_{#1}(#2)}
\newcommand{\efst}[2]{\mathit{efs}_{#1}(#2)}
\newcommand{\tacorres}[3]{\mathit{corres}_{#1}(#2,#3)}
\newcommand{\tacorresb}[5]{\mathit{corres}_{#1}(#2;#3,#4,#5)}
\newcommand{\tabsn}[2]{\mathit{bsn}(#1)_{#2}}
\newcommand{\sbainv}[3]{\mathit{sbainv}_{#1}(#2,#3)}
\newcommand{\bce}[5]{#2\equiv_{#1}^{#3,#4}#5}
\newcommand{\staseq}[3]{#2\equiv_{#1}#3}
\newcommand{\binders}[2]{\mathit{binders}(#1)}
\newcommand{\sass}[2]{\mathit{sass}_{#1}(#2)}
\newcommand{\saes}[2]{\mathit{saes}_{#1}(#2)}
\newcommand{\bci}[2]{\mathit{bci}_{#1}(#2)}


==> introduction.tex <==
\section{Introduction}
%
{\em Equirecursive types\/} consider a recursive type to be equal to its
unrolling and have no explicit term-level coercions to change a term's
type from the former to the latter or vice versa.  This equality
makes deciding type equality and subtyping more difficult than the
other approach---{\em isorecursive types\/}, in which the types are not equal,
but isomorphic, witnessed by explicit term-level coercions.  Previous
work has built intuition, rules, and polynomial-time decision
procedures for equirecursive types for first-order type systems.
Some work has been done for type systems with parametric polymorphism,
but that work is incomplete (see below).  This chapter will give an
intuitive theory of equirecursive types for second-order type systems,
sound and complete rules, and a decision procedure for subtyping.

Another interesting feature of type systems turns out to be quite
related to equirecursive types.  Canning
\etal~\cite{cchmo:F-bounded-quantification} introduced the idea of
{\em F-bounded polymorphism\/}.  In this form of polymorphism a type
bound can mention the type being bounded.  For example, it can require
a type that has a method that returns an object of the type being
bounded.  This form of bound is useful for binary methods and in
typing object encodings~\cite{oce-oopsla}.  Treating a type variable
as being a subtype of its bound when that bound can refer to it is
like treating a recursive type as being equal to its unrolling, and
similar issues arise to formalising such type systems.  This chapter
will also treat F-bounded parameteric polymorphism, and give it an
intuitive formalisation, sound and complete set of rules, and decision
procedure for subtyping.

Amadio and Cardelli~\cite{ac:subtyping-recursive-types} were the first
to investigate the equirecursive approach.  They proposed the {\em
tree interpretation\/} of recursive types, which is based on the idea
of repeatedly unrolling recursive types into possibly-infinite trees.
Two types are equal if their corresponding trees are the same;
similarly, subtyping can be defined on trees and lifted to types.
Amadio and Cardelli made these ideas precise, defined a set of rules
for type equality and subtyping that are sound and complete, and
provided an exponential-time decision procedure for equality and
subtyping.  Kozen \etal~\cite{kps:subtyping-recursive-types} reduced
this exponential time to quadratic time, by defining a notion of tree
automata that generate trees just as types do and a construction from
two tree automata that decides equality and subtyping.  Both Amadio
and Cardelli and Kozen \etal worked with first-order type systems.
Colazzo and Ghelli~\cite{cg:subtyping-recursive-types} investigated a
second-order type system with equirecursion.  They gave a coinductive
set of rules for subtyping and a decision procedure, but did not
relate their rules to trees nor show soundness and completeness to any
intuitive model.  In previous work~\cite{tsot-esop,tsot-tr}, I gave a
tree model for second-order systems, a set of rules for equality of
types, showed soundness and completeness of those rules, defined
automata for the trees, and defined a construction on automata that
gives a decision procedure for equality.\footnote{In those papers I
claimed that the algorithm could be made quadratic time.  I have
recently realised that the reasoning was incorrect, and thus that my
papers demonstrated only an exponential-time algorithm.  The arguments
I give latter can be used to make an $O(n^4)$ algorithm from the ones
in my previous work.}  However, I
did not address subtyping.  Gauthier and
Pottier~\cite{gp:numbering-matters} devised an $O(n\log n)$ algorithm
to decide equality of second-order types with equirecursive types by
reducing second-order types to canonical first-order types in a
particular way such that the canonical types are equal exactly when
the original types are equal; their approach also handles entailment
of type equations and type unification problems with the same
complexity.

This chapter investigates a second-order type system with F-bounded
quantifiers and equirecursive types.  First, it defines a notion of
trees that provide an intuitive model for such types and defines an
intuitive notion of subtyping on these trees.  Next, it presents the
types themselves and defines how these map to trees.  Then it presents
a set of type equality and subtyping rules and shows soundness and
completeness of these rules with respect to the tree interpretation.
Finally, it defines a notion of tree automata, how these generate
trees, and a construction that decides subtyping in polynomial time.

Complete definitions and proofs of all the results in this chapter
appear in a companion technical report~\cite{glew:recsub-tr}.

